TOPIQ: A Top-down Approach from Semantics to Distortions for Image Quality Assessment

Image Quality Assessment (IQA) is a fundamental task in computer vision that has witnessed remarkable progress with deep neural networks. Inspired by the characteristics of the human visual system, existing methods typically use a combination of global and local representations (\ie, multi-scale features) to achieve superior performance. However, most of them adopt simple linear fusion of multi-scale features, and neglect their possibly complex relationship and interaction. In contrast, humans typically first form a global impression to locate important regions and then focus on local details in those regions. We therefore propose a top-down approach that uses high-level semantics to guide the IQA network to focus on semantically important local distortion regions, named as \emph{TOPIQ}. Our approach to IQA involves the design of a heuristic coarse-to-fine network (CFANet) that leverages multi-scale features and progressively propagates multi-level semantic information to low-level representations in a top-down manner. A key component of our approach is the proposed cross-scale attention mechanism, which calculates attention maps for lower level features guided by higher level features. This mechanism emphasizes active semantic regions for low-level distortions, thereby improving performance. CFANet can be used for both Full-Reference (FR) and No-Reference (NR) IQA. We use ResNet50 as its backbone and demonstrate that CFANet achieves better or competitive performance on most public FR and NR benchmarks compared with state-of-the-art methods based on vision transformers, while being much more efficient (with only ${\sim}13\%$ FLOPS of the current best FR method). Codes are released at \url{https://github.com/chaofengc/IQA-PyTorch}.

==> tab_computation.tex <==
\begin{table}[t]
\centering
\caption{Comparison of computation complexity with recent methods based on deep neural networks. The input image is resized or cropped according to the corresponding testing protocol.} \label{tab:datasets}
\resizebox{\linewidth}{!}{
\begin{tabular}{clcccc}
% \hline
\toprule
Type & Method &  \# Params. & \# FLOPS & Time (ms) \\ \midrule
\multirow{5}{*}{FR} & LPIPS & & & \\ 
& PieAPP & & & \\
& DISTS & & & \\
& AHIQ & & & \\
& Ours-FR (Resnet50) & \\
\midrule
\multirow{7}{*}{NR} & TReS \\
& MUSIQ & & & \\
& MANIQA & & & \\
& Ours-NR (Resnet50) & & & \\
& Ours-NR (Swin-base) & & & \\
% \hline
\bottomrule
\end{tabular}
}
\end{table}

==> tab_nr_comp_ava.tex <==
\begin{table}[t] \centering
    \caption{Results on SPAQ dataset.} \label{tab:nr_spaq}
    % \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{18pt}
    \begin{tabular}{lcc}
    \toprule
    Method & PLCC & SRCC \\ \midrule
    DIIVINE~\cite{moorthy2011nssdiivine}  &  0.600 & 0.599 \\
    BRISQUE~\cite{2012brisque} & 0.817 & 0.809 \\ 
    ILNIQE~\cite{zhang2015ilniqe} & 0.721 & 0.713 \\ 
    PI~\cite{blau2018pi} & 0.724 & 0.709 \\ 
    \midrule
    \citet{fang2020spaq} & 0.909 & 0.908 \\
    DBCNN~\cite{2020dbcnn} & 0.915 & 0.911 \\ 
    MUSIQ~\cite{ke2021musiq} & \second{0.920} & \second{0.917} \\
    \midrule
    Ours (ResNet50) & \best{0.924} & \best{0.921} \\
    std & $\pm$0.002 & $\pm$0.003 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{table}[t] \centering
    \caption{Results on AVA dataset. $\dagger$ use extra theme labels.} \label{tab:nr_ava}
    \begin{tabular}{llcc}
    \toprule
    Method & Backbone & PLCC & SRCC \\ \midrule
    NIMA~\cite{talebi2018nima} & Inception-v2 & 0.636 & 0.612 \\
    PQR~\cite{zeng2018pqr} & ResNet101 & 0.720 & 0.719 \\ 
    Hosu \etal \cite{mlspf2019} & Inception-v2 & 0.757 & 0.756 \\
    ThemeAware$^\dagger$~\cite{jia2022themeaware} & Inception-v2 & \textcolor{gray}{0.775} & \textcolor{gray}{0.774} \\
    MUSIQ~\cite{ke2021musiq} & ViT-B/32 & 0.726 & 0.738 \\ 
    KD~\cite{hou2022kd} & ResNeXt101 & \second{0.770} & \second{0.770} \\ 
    \midrule
    \multirow{2}{*}{Ours} & ResNet50 & 0.733 & 0.733 \\
    & Swin-base & \best{0.781} & \best{0.781} \\ 
    \bottomrule
    \end{tabular}
\end{table}

